DropLoss for Long-Tail Instance Segmentation

Long-tailed class distributions are prevalent among the practical applications of object detection and instance segmentation. Prior work in long-tail instance segmentation addresses the imbalance of losses between rare and frequent categories by reducing the penalty for a model incorrectly predicting a rare class label. We demonstrate that the rare categories are heavily suppressed by correct background predictions, which reduces the probability for all foreground categories with equal weight. Due to the relative infrequency of rare categories, this leads to an imbalance that biases towards predicting more frequent categories. Based on this insight, we develop DropLoss -- a novel adaptive loss to compensate for this imbalance without a trade-off between rare and frequent categories. With this loss, we show state-of-the-art mAP across rare, common, and frequent categories on the LVIS dataset.

==> 5_ablation_study.tex <==



\begin{figure}[ht]
% \vspace{-20pt}
% \setlength{\abovecaptionskip}{-3pt} 
% \setlength{\belowcaptionskip}{-15pt} 
    \subfigure[]{%
    \includegraphics[height=0.235\textheight]{fig/parteo_rare.png}%
    \label{fig:parteo_rare}%
    }\hspace{0cm}
    \subfigure[]{%
    \includegraphics[height=0.235\textheight]{fig/parteo_common.png}%
    \label{fig:parteo_common}%
    }\hspace{0cm}
    \vspace{-3mm}
  \caption{Comparison between rare, common, and frequent categories AP for baselines and our method. We visualize the trade-off for `rare vs. frequent' and `common vs. frequent' as a Pareto frontier, where the top-right position indicates an ideal trade-off between objectives. DropLoss achieves an improved trade-off between object categories, resulting in higher overall AP.}
  \label{fig:parteo}
\end{figure}


% rare - dinghy, duckling
% common - pelican, goose, gull

\begin{figure}[ht]
% \vspace{-20pt}
% \setlength{\abovecaptionskip}{-3pt} 
% \setlength{\belowcaptionskip}{-15pt} 
    \subfigure[Mask R-CNN]{%
    \includegraphics[height=0.2\textheight]{fig/maskrcnn.jpg}%
    \label{fig:maskrcnn_predict}%
    }\hspace{0cm}
    \subfigure[DropLoss (Ours)]{%
    \includegraphics[height=0.2\textheight]{fig/drop.jpg}%
    \label{fig:drop_predict}%
    }\hspace{0cm}
  \caption{Qualitative results of \subref{fig:maskrcnn_predict} Mask R-CNN baseline and \subref{fig:drop_predict} the proposed DropLoss. Instances with score > 0.5 are shown. DropLoss adaptively removes background proposal losses of rare and common categories to reduce bias towards misclassifying these objects as background. In this case, the \emph{common} category `goose' is misclassified as background in \subref{fig:maskrcnn_predict}, and correctly identified in \subref{fig:drop_predict}. }
  \label{fig:prediction}
\end{figure}

% \begin{table}[]
% \centering
% \caption{Evaluation on LVIS dataset val 0.5 with other methods. (\%). 
% \label{tab:log_}}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{c|cccccccc}
% logarithm base & AP            & AP50          & AP75          & APr           & APc         & APf           & AR            & AP\_bbox      \\ \hline
% 10             & 25.1          & 38            & 26.9          & \textbf{16.3} & \textbf{28} & 24.8          & 33.7          & 24.4          \\
% 20             & 25.1          & \textbf{38.7} & 26.3          & 13.9          & 27.7        & 26.3          & 34.2          & 24.6          \\
% 30             & 24.9          & 38.3          & 26.4          & 13.6          & 27          & 26.9          & 34.1          & 24.6          \\
% 40             &               &               &               &               &             &               &               &               \\
% 50             & 24.8          & 38.3          & 26.2          & 12.3          & 26.8        & 27.4          & 33.8          & 24.7          \\
% 100            & 24.8          & 38.4          & 26.2          & 10.6          & 27.2        & 27.6          & 34.1          & 24.5          \\
% 150            & 24.8          & 38.3          & 26            & 11.3          & 26.5        & 27.9          & 33.8          & 24.3          \\
% 200            & 24.9          & 38.1          & 26.2          & 9.7           & 27.1        & \textbf{28.1} & 33.4          & 24.6          \\ \hline
% DropLoss(Ours) & \textbf{25.5} & \textbf{38.7} & \textbf{27.2} & 13.2          & 27.9        & 27.3          & \textbf{34.8} & \textbf{25.1}
% \end{tabular}%
% }
% \end{table}


\section{Ablation Study}
% \tim{In this section, we do ablation study to analyze the effect of DropLoss. 
% We compare DropLoss with the background equalization loss and fixed drop ratio on the LVIS dataset \cite{GuptaDG19}. First, we use experiment result to analyze that DropLoss get better scores compared with background equalization loss and fixed drop ratio. Second, we use parteo graph to visualize the balance factor between rare, common and frequent categories. We find that DropLoss can achieve better balance in long tail distribution datasets. And the dynamic drop ratio also can help model learn better.
% }
% \Esther{
% We present an ablation study to analyze the performance of DropLoss. We compare with a variation of equalization loss \cite{tan2020eql} which operates on background rather than foreground categories, to validate the usefulness of our dynamic background loss. Additionally, we compare DropLoss with a fixed drop probability against our batch-frequency method. We demonstrate in experimental results that DropLoss performs better than both of these baselines. Long-tail distribution methods incur a trade-off between performance on rare categories and frequent categories. We can quantify this using a Pareto graph, which shows the relationship between performance scores on multi-objective optimization problems. Figure \ref{fig:parteo} demonstrates trade-offs between rare, common and frequent categories for for several methods. We find that DropLoss with dynamic drop ratio achieves a the most optimal balance between class types in the long-tail setting.
% }




\paragraph{Measuring the balance.}
% \tim{The background equalization loss can adjust the weight for rare and common categories. Decreasing the weight can help rare and common categories receive less discouragement gradient. Vice versa, increasing the weight will cause the score decreasing. Hence, we can adjust the logarithm base to adjust the weight. In Table \ref{tab:log_}, we show up the different logarithm base result. The rare and common categories score will increase as the frequent categories score decreasing. Hence, in order to measure the balance effect, we can observe $AP$, $AP_{50}$, $AP_{75}$ and $AR$. We can find that the DropLoss is not the best score in $AP_r$, $AP_c$ and $AP_f$. However, the DropLoss get the best result in $AP$, $AP_{50}$, $AP_{75}$, $AR$ and $AP_{bbox}$. Therefore, we can measure that DropLoss can reach the most stable balance in all of the experiments.
% }

Long-tail distribution methods often involve a trade-off between accuracy on rare, common, and frequent categories, so we wish to quantify this trade-off for various methods. We compare our proposed DropLoss against three baselines: equalization loss \cite{tan2020eql}, background equalization loss, and fixed drop ratio. Equalization loss and DropLoss have no tunable hyperparameters. Background equalization loss has the log base as a tunable hyperparameter. A fixed drop ratio has the drop ratio as a hyperparameter, so these methods may be adjusted to measure the trade-off between object categories. We can use the Pareto Frontier graph from multi-objective optimization to visualize this trade-off, as seen in Figure \ref{fig:parteo}. We observe that for the reweighting methods with tunable hyperparameters, improvement in rare AP$_\mathrm{r}$ or common AP$_\mathrm{c}$ generally leads to a decrease in frequent AP$_\mathrm{f}$. Our proposed DropLoss does not have tunable hyperparameters, but Figure \ref{fig:parteo} demonstrates that DropLoss balances more effectively between AP$_\mathrm{r}$, AP$_\mathrm{c}$ and AP$_\mathrm{f}$, resulting in a higher overall AP than our baselines. 
DropLoss adapts to the sampling distribution so that if a rare category appears in a given batch, its loss is less likely to be dropped. 
However, if a rare category does not appear in a batch, the chance of its loss being dropped is very high. 
This allows the network to dynamically attend to the categories that it sees in a given batch, decreasing drop loss probability selectively for only those categories. 
We postulate that this allows the network to achieve a better overall balance.


% \Esther{
% Our background equalization baseline method adjusts the loss weights for rare and common categories based on batch class distribution. In developing this baseline, we found that it is beneficial to use different weights for different class categories.
% Our weighting function is $min(log_b(\hat{p}_j))$, where $b$ can be tuned to adjust the weight.
% Table \ref{tab:log_} shows the results for several values of $b$. 
% We observe a trade-off between rare, common, and frequent categories as measured by $AP_r$, $AP_c$ and $AP_f$. The overall balance is reflected in the $AP$, $AP_{50}$, $AP_{75}$, and $AR$. 
% While DropLoss does not achieve the highest performance in the indvidual $AP_r$, $AP_c$ and $AP_f$ categories, it achieves the best result in $AP$, $AP_{50}$, $AP_{75}$, $AR$ and $AP_{bbox}$. 
% Therefore DropLoss is able to balance the trade-off more effectively than our baseline methods.
% }

% \paragraph{Measuring the dynamic drop ratio.}
% \tim{In Table \ref{tab:log_}, we show up the different drop ratio can get different performance. Low drop ratio will not influence the score a lot. As the drop ratio increase, the rare and common categories score will increase, but the frequent categories score decreasing. Compare with the dynamic drop ratio, we can find that it can get better performance in $AP$, $AP_{50}$, $AP_{75}$ and $AR$. Thus, it can verify that using dynamic drop ratio can help model drop more useless loss in different time and keep more useful loss in useful time.
% }
% \Esther{We also compare our proposed dynamic drop loss against several variations on fixed drop ratios. 
% As shown in Table \ref{tab:log_}, the fixed drop ratio incurs a trade-off between rare, common, and frequent categories, depending on the value of the drop rate hyperparameter. 
% We find that the dynamic drop loss achieves better overall balance between categories as measured by $AP$, $AP_{50}$, $AP_{75}$ and $AR$. 

% }



% \paragraph{Visualizing the balance}
% \tim{
% DropLoss will drop different ratio according to the data in every batch. In order to revel the dynamic the drop ratio can get better performance, we draw the parteo figure to measure the
% }

\paragraph{Qualitative results.}
Figure \ref{fig:prediction} demonstrates the results on a dense instance segmentation example containing common category ``goose''. Figure \ref{fig:maskrcnn_predict} demonstrates the suppression of less-frequent categories, as most of the geese in this image are classified as background or with low confidence. In contrast, Figure \ref{fig:drop_predict} correctly identifies all geese as foreground, and guesses category ``goose'' with high confidence and other waterbirds with lower confidence. Despite the stochastic removal of rare and common category losses for background proposals, we find that the network does not misclassify background regions as foreground. The distinction between background and foreground is likely less difficult to learn than the distinction between foreground image categories, so reducing background gradients does not appear to significantly affect background/foreground classification. By reducing the suppression of rare and common categories via background predictions, our method allows for rare and common categories to improve prediction scores, decreasing bias towards frequent categories.




==> 7_supplimentary.tex <==
\section{Overview}

In this supplementary material, we provide additional results to complement the primary manuscript. To further validate our method, we conduct an additional comparison in the no-augmentation setting except horizontal flipping. We also include additional qualitative results. We will make the code for all experiments available online for others to fully reproduce our results.

\section{Data augmentation}

We compare our method against others in an additional setting by removing data augmentation except horizontal flipping. The default data augmentation in the Detectron2 object detection framework \cite{wu2019detectron2} is scale jittering \cite{krizhevsky2012imagenet}, in which the input images are randomly resized to enhance detection of objects at different scales. We include this result for completeness, as the equalization \cite{tan2020eql} baseline did not include scale jittering augmentation in their comparisons \cite{tan2020eql}. Under this additional condition, we find that the DropLoss still achieves the best overall performance as shown in Table \ref{tab:LVIS Effectiveness}.

\begin{table}[th!]
\centering
\caption{\textbf{Results without data augmentation.} Comparison between architecture and backbone settings, evaluated on LVIS v0.5 validation set \cite{GuptaDG19}. We compare BCE (binary cross-entropy), EQL (equalization loss) \cite{tan2020eql} and Drop (DropLoss). AP/AR refers to mask AP/AR, and subscripts `r’, `c’, and `f’ refer to rare, common, and frequent categories. 
\label{tab:LVIS Effectiveness}}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccccc}
\hline
Architecture & Backbone & Loss & AP (\%) & AP$_\mathrm{50}$ & AP$_\mathrm{75}$ & AP$_\mathrm{r}$ & AP$_\mathrm{c}$ & AP$_\mathrm{f}$ & AR & AP$_\mathrm{bbox}$ \\ \hline
\multirow{3}{*}{Mask R-CNN} & \multirow{3}{*}{R-50-FPN} & BCE & 21.3 & 33.3 & 22.6 & 5.1 & 21.5 & \textbf{27.6} & 28.3 & 21 \\
 &  & EQL & 23.4 & 36.1 & 24.8 & 9.9 & 24.6 & 27.3 & 30.9 & 23 \\
 &  & Drop (Ours) & \textbf{24.3} & \textbf{37.4} & \textbf{25.6} & \textbf{13.1} & \textbf{26.1} & 26.4 & \textbf{33.4} & \textbf{23.9} \\ \hline
\multirow{3}{*}{Mask R-CNN} & \multirow{3}{*}{R-101-FPN} & BCE & 23.6 & 36.6 & 25 & 6 & 25 & \textbf{29} & 31 & 23.4 \\
 &  & EQL & 25.3 & 38.5 & 26.9 & 10.6 & 27.4 & 28.7 & 33.3 & 25.2 \\
 &  & Drop (Ours) & \textbf{26.2} & \textbf{39.7} & \textbf{27.8} & \textbf{14.3} & \textbf{28.8} & 27.6 & \textbf{35.6} & \textbf{26.2} \\ \hline
\end{tabular}%
}
\end{table}


\section{Qualitative results}

Figure \ref{fig:prediction1} and Figure \ref{fig:prediction2} show additional qualitative comparisons of our method against the Mask R-CNN baseline.
%
Our method consistently recalls more foreground objects due to the rebalancing of discouraging gradients across the category distribution. 
This can be seen in Figure \ref{fig:prediction1} (c-d) where DropLoss more commonly identifies rare category ``pigeon'' as foreground where Mask R-CNN predicts background.
Additionally in Figure \ref{fig:prediction2} (g-h) Mask R-CNN misidentifies common category ``wedding cake'' objects as background or the wrong foreground category despite the objects appearing prominently in the foreground. DropLoss identifies these objects accurately, with several related but inaccurate guesses appearing (``onion'', ``cupcake'', ``whipped cream'').
%
DropLoss tends towards more fine-grained predictions due to the rebalancing of rare and common categories.
This is evident in Figure \ref{fig:prediction2} (a-b) where DropLoss correctly identifies ``parrot'' where Mask R-CNN predicts coarse-grain frequent category ``bird'', and in Figure \ref{fig:prediction1} (c-d) where DropLoss predicts rare category ``pigeon'' and Mask R-CNN again predicts ``bird''. This example show the bias of Mask R-CNN toward more frequent categories, which may impede fine-grained classification.
%
Both methods suffer from inaccurate predictions, as can be seen in the challenging examples of Figure \ref{fig:prediction1} (a-b) and Figure \ref{fig:prediction2} (c-d) where both methods suffer from inaccurate foreground and background classifications. However, DropLoss has a consistent advantage in identifying foreground objects.

\begin{figure}
    \subfigure[Mask R-CNN]{%
    \includegraphics[height=0.2\textheight, width=0.49\textwidth]{fig/baseline/1.jpg}%
    \label{fig:maskrcnn_predict}%
    }\hspace{0cm}
    \subfigure[DropLoss (Ours)]{%
    \includegraphics[height=0.2\textheight, width=0.49\textwidth]{fig/drop/1.jpg}%
    \label{fig:drop_predict}%
    }\hspace{0cm}
    
    \bigskip
    \subfigure[Mask R-CNN]{%
    \includegraphics[height=0.2\textheight, width=0.49\textwidth]{fig/baseline/2.jpg}%
    \label{fig:maskrcnn_predict}%
    }\hspace{0cm}
    \subfigure[DropLoss (Ours)]{%
    \includegraphics[height=0.2\textheight, width=0.49\textwidth]{fig/drop/2.jpg}%
    \label{fig:drop_predict}%
    }\hspace{0cm}
    
    \bigskip
    \subfigure[Mask R-CNN]{%
    \includegraphics[height=0.2\textheight]{fig/baseline/3.jpg}%
    \label{fig:maskrcnn_predict}%
    }\hspace{0cm}
    \subfigure[DropLoss (Ours)]{%
    \includegraphics[height=0.2\textheight]{fig/drop/3.jpg}%
    \label{fig:drop_predict}%
    }\hspace{0cm}
    
    % \bigskip
    % \subfigure[Mask R-CNN]{%
    % \includegraphics[height=0.2\textheight]{fig/baseline/4.jpg}%
    % \label{fig:maskrcnn_predict}%
    % }\hspace{0cm}
    % \subfigure[DropLoss (Ours)]{%
    % \includegraphics[height=0.2\textheight]{fig/drop/4.jpg}%
    % \label{fig:drop_predict}%
    % }\hspace{0cm}


  \caption{\textbf{Qualitative results.} Visual results of (a,c,e) Mask R-CNN baseline and (b,d,f) the proposed DropLoss. Instances with score > 0.5 are shown. DropLoss adaptively removes background proposal losses of rare and common categories to reduce bias towards misclassifying these objects as background. Rare and common categories pictured include (a)-(b) ``green bean'', ``peach''  (c-d) ``pigeon'', ``bull'', ``tank (storage vessel)'', (e-f) ``gravestone''.}
  \label{fig:prediction1}
\end{figure}

% green bean, peach: rare
% pigeons: rare
% gravestone: common
% wedding cake: common
% calf: common
% bandanna: common
% trunk: common
% basket: frequent
% deer: common
% bull: common
% tank (storage vessel): common
% bird: frequent

\begin{figure}
    \subfigure[Mask R-CNN]{%
    \includegraphics[height=0.2\textheight, width=0.49\textwidth]{fig/baseline/8.jpg}%
    \label{fig:maskrcnn_predict1}%
    }\hspace{0cm}
    \subfigure[DropLoss (Ours)]{%
    \includegraphics[height=0.2\textheight, width=0.49\textwidth]{fig/drop/8.jpg}%
    \label{fig:drop_predict}%
    }\hspace{0cm}
    
    \bigskip
    \subfigure[Mask R-CNN]{%
    \includegraphics[height=0.2\textheight, width=0.49\textwidth]{fig/baseline/9.jpg}%
    \label{fig:maskrcnn_predict2}%
    }\hspace{0cm}
    \subfigure[DropLoss (Ours)]{%
    \includegraphics[height=0.2\textheight, width=0.49\textwidth]{fig/drop/9.jpg}%
    \label{fig:drop_predict}%
    }\hspace{0cm}
    
    \bigskip
    \subfigure[Mask R-CNN]{%
    \includegraphics[height=0.2\textheight, width=0.49\textwidth]{fig/baseline/7.jpg}%
    \label{fig:maskrcnn_predict3}%
    }\hspace{0cm}
    \subfigure[DropLoss (Ours)]{%
    \includegraphics[height=0.2\textheight, width=0.49\textwidth]{fig/drop/7.jpg}%
    \label{fig:drop_predict}%
    }\hspace{0cm}
    
    \bigskip
    \subfigure[Mask R-CNN]{%
    \includegraphics[height=0.2\textheight, width=0.49\textwidth]{fig/baseline/4.jpg}%
    \label{fig:maskrcnn_predict4}%
    }\hspace{0cm}
    \subfigure[DropLoss (Ours)]{%
    \includegraphics[height=0.2\textheight, width=0.49\textwidth]{fig/drop/4.jpg}%
    \label{fig:drop_predict}%
    }\hspace{0cm}


  \caption{\textbf{Qualitative results.} Visual results of (a,c,e,g) Mask R-CNN \cite{he2017mask} baseline and (b,d,f,h) the proposed DropLoss. Instances with score > 0.5 are shown. DropLoss adaptively removes background proposal losses of rare and common categories to reduce bias towards misclassifying these objects as background. Rare and common categories pictured include (a-b) ``parrot'', (c-d) ``beef'', ``crisp (potato chip)'', (e-f) ``pottery'', (g-h) ``wedding cake'', ``bandanna'', ``trunk''.}
  \label{fig:prediction2}
\end{figure}

